Maximizing Data Rate for Multiway Relay Channels with Pairwise Transmission Strategy

In a multiway relay channel (MWRC), pairwise transmission strategy can be used to reduce the computational complexity at the relay and the users without sacrificing the data rate, significantly. The performance of such pairwise strategies, however, is affected by the way that the users are paired to transmit. In this paper, we study the effect of pairing on the common rate and sum rate of an MWRC with functional-decode-forward (FDF) relaying strategy where users experience asymmetric channel conditions. To this end, we first develop a graphical model for an MWRC with pairwise transmission strategy. Using this model, we then find the maximum achievable common rate and sum rate as well as the user pairings that achieve these rates. This marks the ultimate performance of FDF relaying in an MWRC setup. Further, we show that the rate enhancement achieved through the optimal user pairing becomes less pronounced at higher SNRs. Using computer simulations, the performance of the optimal pairing is compared with those of other proposed pairings in the literature.

==> CDFCR.tex <==
\section{Proof of Theorem \ref{CDFCR}}\label{appCDFCR}
We prove the theorem by contradiction. Assume that the ordering $O$ given by (\ref{CDFCRO}) is not optimal and there is another ordering $O'$ that has a higher $C_R$, i.e., $C_R(O') > C_R(O)$.
Assume that 
\begin{equation}
C_R(O) = \frac{1}{4(N-1)}\log_2\left(1+ \gamma_{b(N-i)+1} + \gamma_{N-i}\right)
\end{equation}
for an $i$ such that $m \geq i \geq 1$.
Then, according to the monotonicity of columns of $W$ in (\ref{weightDF}), $U_i$ can be paired with any of $\{U_j|j<N-i\}$ in $O'$.
Monotonicity of rows and columns of $W$ also implies that none of the $U_j$'s for $j \in \{1,2, \dots, i-1\}$, can be paired with $U_k$ when $k \leq N-i$ in $O'$.
As a result, $G_{O'}$ should be disconnected which contradicts Theorem \ref{th1}.
\hfill$\blacksquare$

==> DFCR.tex <==
\section{Proof of Theorem \ref{UDFCR}}\label{appUDFCR}
We first define an $N\times N$ weight matrix $W= (w_{i,j})$ as
\if@twocolumn
\begin{equation}\label{weightDF}
\begin{split}
&w_{i,j} =\\
&\frac{1}{2(N-1)}\min \left\{\log_2{(1 + \gamma_j)}, \frac{1}{2}\log_2{(1 + \gamma_i + \gamma_j)}\right\}
\end{split}
\end{equation}
\else
\begin{equation}\label{weightDF}
w_{i,j} =
\frac{1}{2(N-1)}\min \left\{\log_2{(1 + \gamma_j)}, \frac{1}{2}\log_2{(1 + \gamma_i + \gamma_j)}\right\}
\end{equation}
\fi
for all pairs of $i$ and $j$ with $i\neq j$ and $w_{i,i}=0$.
According to this definition and our assumption that
\begin{equation}
\gamma_N \geq \gamma_{N-1} \geq \dots \geq \gamma_1 > 0
\end{equation}
$w_{i,j}$ is an increasing function of both $j$ and $i$ with $i \neq j$. For a given client graph $G_O$ with adjacency matrix $\mathcal{A}=(a_{i,j})$, we have
\begin{equation}\label{DFCRGO}
\Rc(G_O) = \min \left\{w_{i,j}|a_{i,j} \neq 0 \right\}.
\end{equation}
The client graph $G_O$ is connected and $\mathcal{A}$ is symmetric. As a result, for every $ i = 1,2, \dots , N-1$, there exist at least one $j$ such that $a_{i,j} = 1$. If we define the minimum value of row $i$ in $W$, with respect to $G_O$, as $r_i = \min \{w_{i,j}|a_{i,j} \neq 0; j = 1, 2, \dots , N\}$ for $ i = 1,2, \dots , N$, and also define the minimum value of column $k$ with respect to $G_O$ as $c_k = \min \{w_{j,k}|a_{j,k} \neq 0; j = 1, 2, \dots , N\}$ for every $ k = 1,2, \dots , N$, we can rewrite equation (\ref{DFCRGO}) as:
\begin{equation}\label{rewrite1}
\Rc(G_O) = \min \left\{c_1, c_2, \dots , c_N\right\}
\end{equation}
and
\begin{equation}\label{rewrite2}
\Rc(G_O) = \min \left\{r_1, r_2, \dots , r_N\right\}.
\end{equation}



The ordering which achieves the maximum $\Rc$ is the one which maximizes the right hand side of equations (\ref{rewrite1}) and (\ref{rewrite2}). However, we know that $c_k \leq w_{N,k}$ and $r_i \leq w_{i,N}$. The ordering $O = \{\{U_1,U_N\},\{U_2,U_N\},\dots ,\{U_{N-1},U_N\}\}$ maximizes both $c_k$s and $r_i$s by picking the most significant entries in each column and each row, simultaneously. Consequently, it achieves the maximum $\Rc$ in a DF MWRC. As a result, the common rate is given by
\begin{equation}\label{inn}
\Rc(G_O) = \min \{w_{1,N}, w_{N,1}\}
\end{equation}
The proof becomes complete by considering the cases that the downlink is the bottleneck of the common rate and (\ref{inn}).
\hfill$\blacksquare$

==> DFSR.tex <==
\section{Proof of Theorem \ref{DFSR}}\label{appDFSR}
We prove Theorem \ref{DFSR} by induction. For $N=2$, $S_R=\frac{1}{2}\log_2\left(1 + \gamma_1 + \gamma_2\right)$ which is true for a two way relay channel with half-duplex DF relaying. Now, assume that the statement of Theorem \ref{DFSR} is true for all $N \leq k$. We show that it also holds for $N=k+1$.
If $deg(v_1) = N - 1$, the statement holds. Otherwise, $deg(v_1) < N-1$.
Let us define $V'$ the set of all neighbors of $v_1$ that have a degree greater than 1, i.e., 
\begin{equation}\label{DFSReqn2}
V' = \{v_j \in A_1^{G_O} | deg(v_j) > 1\}.
\end{equation}
Note that $deg(v_1) < N-1$ and as a result, $V'$ is nonempty.
Since $G_O$ is a tree, there exists one unique path from $v_1$ to any other node $v_i$, $i \neq 1$. We define the set of edges that form a path from $v_1$ to $v_i$ by ${\mathcal{P}}_i$. For any $v_j  \in V'$ and considering $v_1$ as the root of $G_O$, we define  the set of descendants of $v_j$ as $D_j = \{ v_i \in V| v_1v_j \in {\mathcal{P}}_i; i \neq j\}$. Fig. \ref{descendants} illustrates the set of descendants of $v_j$.

\begin{figure}[!h] 
\psfrag{U_1}{$v_1$}
\psfrag{U_2}{}
\psfrag{D_j}{$D_j$}
\psfrag{U_3}{}
\psfrag{U_4}{}
\psfrag{U_j}{$v_{j}$}
\psfrag{v..}{$\vdots$}
\psfrag{...}{$\dots$}
\centering
\includegraphics[scale = 0.3]{DESCENDANTS.eps}
\caption{Set of descendants of $v_j$.}
\label{descendants}
\end{figure}
Since $deg(v_1) < N-1$, there exists at least one $j$ such that $D_j \neq \{\}$. For these $j$'s, we define the highest SNR among the descendant of $v_j$ and $v_j$ itself, as
\begin{equation}\label{DFSReqn3}
h^*(v_j) = \max \{\gamma_i| v_i \in D_j \cup {v_j}\}.
\end{equation} 
Now, assume that 
\begin{equation}\label{DFSReqn4}
v^* = \operatorname*{arg\,max}_{v_j \in A_1^{G_O}, D_j \neq \{\}} h^*(v_j).
\end{equation}
We denote the set of descendants of $v^*$ by $D^*$. According to the induction hypothesis, by removing $v^*$ and all of its descendants from the client tree $G_O$, we have
\if@twocolumn
\begin{equation}\label{ind1}
\begin{split}
&R_1 + \sum_{v_i \in A_1^{G_O} - \{v^*\}}R_i\\
&\leq \frac{1}{2(N-1)}\log_2\left( \frac{(1+\gamma_1)\times \prod_{v_i\in A_1^{G_O} - \{v^*\}}{(1+\gamma_i)}}{1+ \frac{\gamma_1\gamma_1^*}{1+\gamma_1 + \gamma_1^*}} \right)
\end{split}
\end{equation}
\else
\begin{equation}\label{ind1}
R_1 + \sum_{v_i \in A_1^{G_O} - \{v^*\}}R_i
\leq \frac{1}{2(N-1)}\log_2\left( \frac{(1+\gamma_1)\times \prod_{v_i\in A_1^{G_O} - \{v^*\}}{(1+\gamma_i)}}{1+ \frac{\gamma_1\gamma_1^*}{1+\gamma_1 + \gamma_1^*}} \right)
\end{equation}
\fi
where, $\gamma_1^* = \max \{\gamma_i|v_i \in A_1^{G_O} - \{v^*\}\}$.
Similarly, by removing $v_1$ and all of its neighbors, except $v^*$, we have 
\if@twocolumn
\begin{equation}\label{ind2}
\begin{split}
&\sum_{v_i \in D^* \cup {v^*}}{R_i} \leq\\
&\frac{1}{2(N-1)}\log_2\left(\frac{(1+h^*(v^*)) \times \prod_{{v_i \in D^*}}{(1+\gamma_i)}}{1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}}\right)
\end{split}
\end{equation}
\else
\begin{equation}\label{ind2}
\sum_{v_i \in D^* \cup {v^*}}{R_i} \leq
\frac{1}{2(N-1)}\log_2\left(\frac{(1+h^*(v^*)) \times \prod_{{v_i \in D^*}}{(1+\gamma_i)}}{1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}}\right)
\end{equation}
\fi
where, $\gamma_\mathrm{min} = \min \{\gamma_i|v_i \in D^* \cup \{v^*\}\}$. Now, we have $\gamma_N = \max \{h^*(v^*), \gamma_1^*\}$ and $\gamma_1 \leq \gamma_{\mathrm{min}}$.
Then, as a result of (\ref{DF_rate_i}),(\ref{ind1}) and (\ref{ind2}), we have
\if@twocolumn
\begin{equation}
\begin{split}
&\sum_{i = 1}^{N}{R_i} \leq\\
&\frac{1}{2(N-1)}\log_2\left(\frac{\prod_{i=1}^N{(1+\gamma_i)}}{\left(1+\frac{\gamma_1 \times \gamma_1^*}{1 + \gamma_1 + \gamma_1^*}\right)\left(1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}\right)}\right).
\end{split}
\end{equation}
\else
\begin{equation}
\sum_{i = 1}^{N}{R_i} \leq
\frac{1}{2(N-1)}\log_2\left(\frac{\prod_{i=1}^N{(1+\gamma_i)}}{\left(1+\frac{\gamma_1 \times \gamma_1^*}{1 + \gamma_1 + \gamma_1^*}\right)\left(1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}\right)}\right).
\end{equation}
\fi
This configuration achieves a lower sum rate than (\ref{maxDFSR}) iff
\if@twocolumn
\begin{equation}
\begin{split}
\left(1+\frac{\gamma_1 \times \gamma_1^*}{1 + \gamma_1 + \gamma_1^*}\right)\left(1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}\right) &\geq\\ \left(1+\frac{\gamma_1\gamma_N}{1 + \gamma_1 + \gamma_N}\right)&
\end{split}
\end{equation}
\else
\begin{equation}
\left(1+\frac{\gamma_1 \times \gamma_1^*}{1 + \gamma_1 + \gamma_1^*}\right)\left(1+\frac{\gamma_{\mathrm{min}} \times h^*(v^*)}{1 + \gamma_{\mathrm{min}} + h^*(v^*)}\right) \geq \left(1+\frac{\gamma_1\gamma_N}{1 + \gamma_1 + \gamma_N}\right)
\end{equation}
\fi
which, according to the fact that $\gamma_N = \max \{h^*(v^*), \gamma_1^*\}$, is true.
\hfill$\blacksquare$


==> DFbar.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{0}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6.5}{5}\selectfont\strut}%
\psfrag{054}[cl][cl]{\matlabtextC Cut-set bound}%
\psfrag{055}[cl][cl]{\matlabtextC Optimal ordering}%
\psfrag{056}[cl][cl]{\matlabtextC TDM}%
\psfrag{057}[cl][cl]{\matlabtextC Random Ordering}%
\psfrag{058}[tc][tc]{\matlabtextA $N$}%
\psfrag{059}[bc][bc]{\matlabtextB $\Rs$ for DF, High SNR}%
\psfrag{060}[tc][tc]{\matlabtextA $N$}%
\psfrag{061}[bc][bc]{\matlabtextB $\Rc$ for DF, High SNR}%
\psfrag{062}[tc][tc]{\matlabtextA $N$}%
\psfrag{063}[bc][bc]{\matlabtextB $\Rs$ for DF, Low SNR}%
\psfrag{064}[tc][tc]{\matlabtextA $N$}%
\psfrag{065}[bc][bc]{\matlabtextB $\Rc$ for DF, Low SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
\psfrag{015}[ct][ct]{\matlabtextA $2$}%
\psfrag{016}[ct][ct]{\matlabtextA $4$}%
\psfrag{017}[ct][ct]{\matlabtextA $6$}%
\psfrag{018}[ct][ct]{\matlabtextA $8$}%
\psfrag{019}[ct][ct]{\matlabtextA $10$}%
\psfrag{020}[ct][ct]{\matlabtextA $12$}%
\psfrag{021}[ct][ct]{\matlabtextA $14$}%
\psfrag{026}[ct][ct]{\matlabtextA $2$}%
\psfrag{027}[ct][ct]{\matlabtextA $4$}%
\psfrag{028}[ct][ct]{\matlabtextA $6$}%
\psfrag{029}[ct][ct]{\matlabtextA $8$}%
\psfrag{030}[ct][ct]{\matlabtextA $10$}%
\psfrag{031}[ct][ct]{\matlabtextA $12$}%
\psfrag{032}[ct][ct]{\matlabtextA $14$}%
\psfrag{041}[ct][ct]{\matlabtextA $2$}%
\psfrag{042}[ct][ct]{\matlabtextA $4$}%
\psfrag{043}[ct][ct]{\matlabtextA $6$}%
\psfrag{044}[ct][ct]{\matlabtextA $8$}%
\psfrag{045}[ct][ct]{\matlabtextA $10$}%
\psfrag{046}[ct][ct]{\matlabtextA $12$}%
\psfrag{047}[ct][ct]{\matlabtextA $14$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextA $0$}%
\psfrag{008}[rc][rc]{\matlabtextA $1$}%
\psfrag{009}[rc][rc]{\matlabtextA $2$}%
\psfrag{010}[rc][rc]{\matlabtextA $3$}%
\psfrag{011}[rc][rc]{\matlabtextA $4$}%
\psfrag{012}[rc][rc]{\matlabtextA $5$}%
\psfrag{013}[rc][rc]{\matlabtextA $6$}%
\psfrag{014}[rc][rc]{\matlabtextA $7$}%
\psfrag{022}[rc][rc]{\matlabtextA $0$}%
\psfrag{023}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{024}[rc][rc]{\matlabtextA $1$}%
\psfrag{025}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{033}[rc][rc]{\matlabtextA $0$}%
\psfrag{034}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{035}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{036}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{037}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{038}[rc][rc]{\matlabtextA $1$}%
\psfrag{039}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{040}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{048}[rc][rc]{\matlabtextA $0$}%
\psfrag{049}[rc][rc]{\matlabtextA $0.05$}%
\psfrag{050}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{051}[rc][rc]{\matlabtextA $0.15$}%
\psfrag{052}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{053}[rc][rc]{\matlabtextA $0.25$}%
%
%% </ytick>

==> DFbar2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{10}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{1}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{12}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{5.5}{5}\selectfont\strut}%
\psfrag{054}[cl][cl]{\matlabtextD Cut-set bound}%
\psfrag{055}[cl][cl]{\matlabtextD Optimal ordering}%
\psfrag{056}[cl][cl]{\matlabtextD TDM}%
\psfrag{057}[cl][cl]{\matlabtextD Random Ordering}%
\psfrag{058}[tc][tc]{\matlabtextC $N$}%
\psfrag{059}[bc][bc]{\matlabtextB $\Rs$ for DF, High SNR}%
\psfrag{060}[tc][tc]{\matlabtextC $N$}%
\psfrag{061}[bc][bc]{\matlabtextB $\Rc$ for DF, High SNR}%
\psfrag{062}[tc][tc]{\matlabtextC $N$}%
\psfrag{063}[bc][bc]{\matlabtextB $\Rs$ for DF, Low SNR}%
\psfrag{064}[tc][tc]{\matlabtextC $N$}%
\psfrag{065}[bc][bc]{\matlabtextB $\Rc$ for DF, Low SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
\psfrag{015}[ct][ct]{\matlabtextA $2$}%
\psfrag{016}[ct][ct]{\matlabtextA $4$}%
\psfrag{017}[ct][ct]{\matlabtextA $6$}%
\psfrag{018}[ct][ct]{\matlabtextA $8$}%
\psfrag{019}[ct][ct]{\matlabtextA $10$}%
\psfrag{020}[ct][ct]{\matlabtextA $12$}%
\psfrag{021}[ct][ct]{\matlabtextA $14$}%
\psfrag{026}[ct][ct]{\matlabtextA $2$}%
\psfrag{027}[ct][ct]{\matlabtextA $4$}%
\psfrag{028}[ct][ct]{\matlabtextA $6$}%
\psfrag{029}[ct][ct]{\matlabtextA $8$}%
\psfrag{030}[ct][ct]{\matlabtextA $10$}%
\psfrag{031}[ct][ct]{\matlabtextA $12$}%
\psfrag{032}[ct][ct]{\matlabtextA $14$}%
\psfrag{041}[ct][ct]{\matlabtextA $2$}%
\psfrag{042}[ct][ct]{\matlabtextA $4$}%
\psfrag{043}[ct][ct]{\matlabtextA $6$}%
\psfrag{044}[ct][ct]{\matlabtextA $8$}%
\psfrag{045}[ct][ct]{\matlabtextA $10$}%
\psfrag{046}[ct][ct]{\matlabtextA $12$}%
\psfrag{047}[ct][ct]{\matlabtextA $14$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextA $0$}%
\psfrag{008}[rc][rc]{\matlabtextA $1$}%
\psfrag{009}[rc][rc]{\matlabtextA $2$}%
\psfrag{010}[rc][rc]{\matlabtextA $3$}%
\psfrag{011}[rc][rc]{\matlabtextA $4$}%
\psfrag{012}[rc][rc]{\matlabtextA $5$}%
\psfrag{013}[rc][rc]{\matlabtextA $6$}%
\psfrag{014}[rc][rc]{\matlabtextA $7$}%
\psfrag{022}[rc][rc]{\matlabtextA $0$}%
\psfrag{023}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{024}[rc][rc]{\matlabtextA $1$}%
\psfrag{025}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{033}[rc][rc]{\matlabtextA $0$}%
\psfrag{034}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{035}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{036}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{037}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{038}[rc][rc]{\matlabtextA $1$}%
\psfrag{039}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{040}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{048}[rc][rc]{\matlabtextA $0$}%
\psfrag{049}[rc][rc]{\matlabtextA $0.05$}%
\psfrag{050}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{051}[rc][rc]{\matlabtextA $0.15$}%
\psfrag{052}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{053}[rc][rc]{\matlabtextA $0.25$}%
%
%% </ytick>

==> FDFbar2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{10}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{1}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{12}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{5.5}{5}\selectfont\strut}%
\psfrag{056}[cl][cl]{\matlabtextD Cut-set bound}%
\psfrag{057}[cl][cl]{\matlabtextD Optimal ordering}%
\psfrag{058}[cl][cl]{\matlabtextD TDM}%
\psfrag{059}[cl][cl]{\matlabtextD Ordering of \cite{Parastoo}}%
\psfrag{060}[cl][cl]{\matlabtextD Random ordering}%
\psfrag{061}[tc][tc]{\matlabtextC $N$}%
\psfrag{062}[bc][bc]{\matlabtextB $\Rs$ for FDF, High SNR}%
\psfrag{063}[tc][tc]{\matlabtextC $N$}%
\psfrag{064}[bc][bc]{\matlabtextB $\Rc$ for FDF, High SNR}%
\psfrag{065}[tc][tc]{\matlabtextC $N$}%
\psfrag{066}[bc][bc]{\matlabtextB $\Rs$ for FDF, Low SNR}%
\psfrag{067}[tc][tc]{\matlabtextC $N$}%
\psfrag{068}[bc][bc]{\matlabtextB $\Rc$ for FDF, Low SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
\psfrag{015}[ct][ct]{\matlabtextA $2$}%
\psfrag{016}[ct][ct]{\matlabtextA $4$}%
\psfrag{017}[ct][ct]{\matlabtextA $6$}%
\psfrag{018}[ct][ct]{\matlabtextA $8$}%
\psfrag{019}[ct][ct]{\matlabtextA $10$}%
\psfrag{020}[ct][ct]{\matlabtextA $12$}%
\psfrag{021}[ct][ct]{\matlabtextA $14$}%
\psfrag{026}[ct][ct]{\matlabtextA $2$}%
\psfrag{027}[ct][ct]{\matlabtextA $4$}%
\psfrag{028}[ct][ct]{\matlabtextA $6$}%
\psfrag{029}[ct][ct]{\matlabtextA $8$}%
\psfrag{030}[ct][ct]{\matlabtextA $10$}%
\psfrag{031}[ct][ct]{\matlabtextA $12$}%
\psfrag{032}[ct][ct]{\matlabtextA $14$}%
\psfrag{041}[ct][ct]{\matlabtextA $2$}%
\psfrag{042}[ct][ct]{\matlabtextA $4$}%
\psfrag{043}[ct][ct]{\matlabtextA $6$}%
\psfrag{044}[ct][ct]{\matlabtextA $8$}%
\psfrag{045}[ct][ct]{\matlabtextA $10$}%
\psfrag{046}[ct][ct]{\matlabtextA $12$}%
\psfrag{047}[ct][ct]{\matlabtextA $14$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextA $0$}%
\psfrag{008}[rc][rc]{\matlabtextA $1$}%
\psfrag{009}[rc][rc]{\matlabtextA $2$}%
\psfrag{010}[rc][rc]{\matlabtextA $3$}%
\psfrag{011}[rc][rc]{\matlabtextA $4$}%
\psfrag{012}[rc][rc]{\matlabtextA $5$}%
\psfrag{013}[rc][rc]{\matlabtextA $6$}%
\psfrag{014}[rc][rc]{\matlabtextA $7$}%
\psfrag{022}[rc][rc]{\matlabtextA $0$}%
\psfrag{023}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{024}[rc][rc]{\matlabtextA $1$}%
\psfrag{025}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{033}[rc][rc]{\matlabtextA $0$}%
\psfrag{034}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{035}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{036}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{037}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{038}[rc][rc]{\matlabtextA $1$}%
\psfrag{039}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{040}[rc][rc]{\matlabtextA $1.4$}%
\psfrag{048}[rc][rc]{\matlabtextA $0$}%
\psfrag{049}[rc][rc]{\matlabtextA $0.05$}%
\psfrag{050}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{051}[rc][rc]{\matlabtextA $0.15$}%
\psfrag{052}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{053}[rc][rc]{\matlabtextA $0.25$}%
\psfrag{054}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{055}[rc][rc]{\matlabtextA $0.35$}%
%
%% </ytick>

==> Fig_CR_DF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{5}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6.5}{5}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{35}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{15}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA TDM}%
\psfrag{022}[cl][cl]{\matlabtextC Random ordering}%
\psfrag{023}[cl][cl]{\matlabtextC Optimal ordering}%
\psfrag{024}[cl][cl]{\matlabtextC Upper bound}%
\psfrag{025}[bc][bc]{\matlabtextB $\Rc$ {\tiny(bits of information per round of full data exchange)}}%
\psfrag{026}[tc][tc]{\matlabtextD $1/\sigma^2 $ (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $4$}%
\psfrag{003}[ct][ct]{\matlabtextA $6$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
\psfrag{005}[ct][ct]{\matlabtextA $10$}%
\psfrag{006}[ct][ct]{\matlabtextA $12$}%
\psfrag{007}[ct][ct]{\matlabtextA $14$}%
\psfrag{008}[ct][ct]{\matlabtextA $16$}%
\psfrag{009}[ct][ct]{\matlabtextA $18$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextA $0$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{015}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{016}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{018}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{019}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{020}[rc][rc]{\matlabtextA $0.9$}%
%
%% </ytick>

==> Fig_CR_FDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{5}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6.5}{5}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{35}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{15}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextC Ordering proposed in \cite{Parastoo}}%
\psfrag{023}[cl][cl]{\matlabtextC TDM}%
\psfrag{024}[cl][cl]{\matlabtextC Random ordering}%
\psfrag{025}[cl][cl]{\matlabtextC Optimal ordering}%
\psfrag{026}[cl][cl]{\matlabtextC Upper bound}%
\psfrag{027}[bc][bc]{\matlabtextB $\Rc$ {\tiny(bits of information per round of full data exchange)}}%
\psfrag{028}[tc][tc]{\matlabtextD $1/\sigma^2 $ (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $4$}%
\psfrag{003}[ct][ct]{\matlabtextA $6$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
\psfrag{005}[ct][ct]{\matlabtextA $10$}%
\psfrag{006}[ct][ct]{\matlabtextA $12$}%
\psfrag{007}[ct][ct]{\matlabtextA $14$}%
\psfrag{008}[ct][ct]{\matlabtextA $16$}%
\psfrag{009}[ct][ct]{\matlabtextA $18$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextA $0$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{015}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{016}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{018}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{019}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{020}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{021}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>

==> Fig_SR_DF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{5}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6.5}{5}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{35}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{15}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextC TDM}%
\psfrag{022}[cl][cl]{\matlabtextC Random ordering}%
\psfrag{023}[cl][cl]{\matlabtextC Optimal ordering}%
\psfrag{024}[cl][cl]{\matlabtextC Upper bound}%
\psfrag{025}[bc][bc]{\matlabtextB $\Rs$ {\tiny(bits of information per round of full data exchange)}}%
\psfrag{026}[tc][tc]{\matlabtextD $1/\sigma^2 $ (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $4$}%
\psfrag{003}[ct][ct]{\matlabtextA $6$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
\psfrag{005}[ct][ct]{\matlabtextA $10$}%
\psfrag{006}[ct][ct]{\matlabtextA $12$}%
\psfrag{007}[ct][ct]{\matlabtextA $14$}%
\psfrag{008}[ct][ct]{\matlabtextA $16$}%
\psfrag{009}[ct][ct]{\matlabtextA $18$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextA $0$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextA $2$}%
\psfrag{016}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $3$}%
\psfrag{018}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{019}[rc][rc]{\matlabtextA $4$}%
\psfrag{020}[rc][rc]{\matlabtextA $4.5$}%
%
%% </ytick>

==> Fig_SR_FDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{5}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6.5}{5}\selectfont\strut}%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{35}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{15}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextC Ordering proposed in \cite{Parastoo}}%
\psfrag{022}[cl][cl]{\matlabtextC TDM}%
\psfrag{023}[cl][cl]{\matlabtextC Random ordering}%
\psfrag{024}[cl][cl]{\matlabtextC Optimal ordering}%
\psfrag{025}[cl][cl]{\matlabtextC Upper bound}%
\psfrag{026}[bc][bc]{\matlabtextB $\Rs$ {\tiny(bits of information per round of full data exchange)}}%
\psfrag{027}[tc][tc]{\matlabtextD $1/\sigma^2 $ (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $4$}%
\psfrag{003}[ct][ct]{\matlabtextA $6$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
\psfrag{005}[ct][ct]{\matlabtextA $10$}%
\psfrag{006}[ct][ct]{\matlabtextA $12$}%
\psfrag{007}[ct][ct]{\matlabtextA $14$}%
\psfrag{008}[ct][ct]{\matlabtextA $16$}%
\psfrag{009}[ct][ct]{\matlabtextA $18$}%
\psfrag{010}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextA $0$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextA $1$}%
\psfrag{014}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextA $2$}%
\psfrag{016}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{017}[rc][rc]{\matlabtextA $3$}%
\psfrag{018}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{019}[rc][rc]{\matlabtextA $4$}%
\psfrag{020}[rc][rc]{\matlabtextA $4.5$}%
%
%% </ytick>
